Revisiting the Uniform Information Density Hypothesis in LLM Reasoning

The Uniform Information Density (UID) hypothesis proposes that effective communication is achieved by maintaining a stable flow of information. In this work, we revisit this principle in the context of Large Language Model (LLM) reasoning, asking whether step-level uniformity reflects reasoning quality. To this end, we introduce a novel framework to quantify uniformity of information flow at both local and global levels, using an entropy-based stepwise density metric. Across experiments on seven reasoning benchmarks, we see a counter-intuitive pattern: while high-quality reasoning exhibit smooth step-by-step transitions local uniformity and structured, non-uniform information flow at the trajectory level global non-uniformity. The results demonstrate that these uniformities outperform alternative internal signals as predictors of reasoning quality, and such divergence with human communication is not a model deficiency, but a byproduct of distinct objectives between human communication and LLM reasoning.

==> Tables/StepTokenSeed_Qwen3.tex <==
% put this once in the preamble (or before the table)
\renewcommand{\pmfs}[1]{\,$\pm$\text{\footnotesize #1}}

\begin{table*}[t]
\caption{\textbf{Fixed Window Segmentation.} Results of \texttt{Qwen3-8B} models on AIME, HMMT, BRUMO. Performance is reported across seeds 42, 1234, and 2025, with averages and standard deviations (Avg~$\pm$~Std).}
\label{tab:scalemodelseed}
\centering
\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{@{}l|cccc|cccc|cccc@{}}
\toprule
\multirow{2}{*}{Methods ($\downarrow$)} &
\multicolumn{4}{c|}{AIME} &
\multicolumn{4}{c|}{HMMT} &
\multicolumn{4}{c}{BRUMO} \\ \cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
 & {42} & {1234} & {2025} & {Avg $\pm$ Std}
 & {42} & {1234} & {2025} & {Avg $\pm$ Std}
 & {42} & {1234} & {2025} & {Avg $\pm$ Std} \\ \midrule
Mean Acc. 
&  &  &  & 
&  &  &  & 
&  &  &  &  \\
Self-Cert. 
&  &  &  & 
&  &  &  & 
&  &  &  &  \\
High Conf. 
&  &  &  & 
&  &  &  & 
&  &  &  &  \\
Low Ent. 
&  &  &  & 
&  &  &  & 
&  &  &  &  \\
\midrule
UID Metrics ($\downarrow$) \\
\midrule
Loc. non-uni (3$\sigma$) 
&  &  &  & 
&  &  &  & 
&  &  &  &  \\
\rowcolor{lightblue}
Loc. uni (3$\sigma$) 
&  &  &  & 
&  &  &  & 
&  &  &  &  \\
\rowcolor{lightblue}
Glob. non-uni 
&  &  &  & 
&  &  &  & 
&  &  &  &  \\
Glob. uni 
&  &  &  & 
&  &  &  & 
&  &  &  &  \\
\bottomrule
\end{tabular}%
}
\end{table*}

